Preliminary Results Towards Contract Monitorability

This paper discusses preliminary investigations on the monitorability of contracts for web service descriptions. There are settings where servers do not guarantee statically whether they satisfy some specified contract, which forces the client (i.e., the entity interacting with the server) to perform dynamic checks. This scenario may be viewed as an instance of Runtime Verification, where a pertinent question is whether contracts can be monitored for adequately at runtime, otherwise stated as the monitorability of contracts. We consider a simple language of finitary contracts describing both clients and servers, and develop a formal framework that describes server contract monitoring. We define monitor properties that potentially contribute towards a comprehensive notion of contract monitorability and show that our simple contract language satisfies these properties.

==> eptcsdata.tex <==
\providecommand{\firstpage}{54}
\providecommand{\publicationstatus}{L. Aceto, A. Francalanza and A. Ingolfsdottir (Eds.):  Workshop on \\ Pre- and Post-Deployment Verification Techniques (PrePost 2016)\\
EPTCS 208, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.208.5}{10.4204/EPTCS.208.5}}

